CTRL: Concurrent Training and Rollout for LLM Reinforcement Learning via GPU Co-Residency

Reinforcement learning (RL) post-training of large language models runs two GPU workloads with different hardware demands: rollout decoding, which is dominated by memory access and whose batch shrinks as responses finish, and a dense learner. Current systems either time-share every GPU between them, paying serial phases and switches, or split GPUs into pools whose sizes change only in whole devices. We present CTRL, which makes co-residency a third RL execution layout: every GPU runs a learner rank beside a persistent rollout engine, sharing the device under CUDA MPS. A host-owned learner makes the layout fit: optimizer state stays in host memory, and policy weights stream layer by layer through a bounded GPU window. A publication gate trains each ready batch first and waits only before releasing the next policy, keeping a dropless staleness bound. A step-time bound guides compute-share selection, and a GPU-time ledger explains overlap and sharing costs. On H100, A800, and RTX 4090 GPUs with Qwen3 models, CTRL achieves 1.11-2.24$\times$ the throughput of the stronger of verl's asynchronous baselines across 24 workload settings with the staleness limit set to two, and 1.23$\times$ verl's colocate_async on eight H100 GPUs. With the same learner, co-residency is 1.10-1.26$\times$ faster than time-sharing on all three platforms and 1.10-1.30$\times$ faster than the best measured whole-GPU split on H100 DAPO-Math workloads at 256-528 trajectories per step, on four and eight GPUs.

==> tables/numbers-final.tex <==
\makeatletter
\newcommand{\fm}[2]{\ifcsname fm@#1@#2\endcsname\csname fm@#1@#2\endcsname\else\pendingnote{TBD}\fi}
\newcommand{\fmx}[2]{\ifcsname fmx@#1@#2\endcsname\csname fmx@#1@#2\endcsname\else\pendingnote{TBD}\fi}
\newcommand{\fmb}[1]{\ifcsname fmb@#1\endcsname\csname fmb@#1\endcsname\else\pendingnote{TBD}\fi}
\newcommand{\fmdc}[1]{\ifcsname fmdc@#1\endcsname\csname fmdc@#1\endcsname\else\pendingnote{TBD}\fi}
\newcommand{\fmds}[1]{\ifcsname fmds@#1\endcsname\csname fmds@#1\endcsname\else\pendingnote{TBD}\fi}
\newcommand{\fmg}[1]{\ifcsname fmg@#1\endcsname\csname fmg@#1\endcsname\else\pendingnote{TBD}\fi}
\expandafter\def\csname fm@r8b64@sync\endcsname{626}
\expandafter\def\csname fm@r8b64@colocate_async\endcsname{777}
\expandafter\def\csname fm@r8b64@async_2p2\endcsname{755}
\expandafter\def\csname fm@r8b64@ctrl\endcsname{1053}
\expandafter\def\csname fmx@r8b64@sync\endcsname{1.68}
\expandafter\def\csname fmx@r8b64@colocate_async\endcsname{1.35}
\expandafter\def\csname fmx@r8b64@async_2p2\endcsname{1.39}
\expandafter\def\csname fmb@r8b64\endcsname{1.35}
\expandafter\def\csname fmdc@r8b64\endcsname{1.14}
\expandafter\def\csname fmds@r8b64\endcsname{1.19}
\expandafter\def\csname fmg@r8b64\endcsname{45}
\expandafter\def\csname fm@r8b128@sync\endcsname{876}
\expandafter\def\csname fm@r8b128@colocate_async\endcsname{1150}
\expandafter\def\csname fm@r8b128@async_2p2\endcsname{961}
\expandafter\def\csname fm@r8b128@ctrl\endcsname{1687}
\expandafter\def\csname fmx@r8b128@sync\endcsname{1.93}
\expandafter\def\csname fmx@r8b128@colocate_async\endcsname{1.47}
\expandafter\def\csname fmx@r8b128@async_2p2\endcsname{1.76}
\expandafter\def\csname fmb@r8b128\endcsname{1.47}
\expandafter\def\csname fmdc@r8b128\endcsname{1.31}
\expandafter\def\csname fmds@r8b128\endcsname{1.12}
\expandafter\def\csname fmg@r8b128\endcsname{42}
\expandafter\def\csname fm@r8b256@sync\endcsname{1199}
\expandafter\def\csname fm@r8b256@colocate_async\endcsname{1457}
\expandafter\def\csname fm@r8b256@async_2p2\endcsname{1247}
\expandafter\def\csname fm@r8b256@ctrl\endcsname{2076}
\expandafter\def\csname fmx@r8b256@sync\endcsname{1.73}
\expandafter\def\csname fmx@r8b256@colocate_async\endcsname{1.42}
\expandafter\def\csname fmx@r8b256@async_2p2\endcsname{1.67}
\expandafter\def\csname fmb@r8b256\endcsname{1.42}
\expandafter\def\csname fmdc@r8b256\endcsname{1.33}
\expandafter\def\csname fmds@r8b256\endcsname{1.07}
\expandafter\def\csname fmg@r8b256\endcsname{24}
\expandafter\def\csname fm@a8b64@sync\endcsname{811}
\expandafter\def\csname fm@a8b64@colocate_async\endcsname{1187}
\expandafter\def\csname fm@a8b64@async_2p2\endcsname{1191}
\expandafter\def\csname fm@a8b64@ctrl\endcsname{1511}
\expandafter\def\csname fmx@a8b64@sync\endcsname{1.86}
\expandafter\def\csname fmx@a8b64@colocate_async\endcsname{1.27}
\expandafter\def\csname fmx@a8b64@async_2p2\endcsname{1.27}
\expandafter\def\csname fmb@a8b64\endcsname{1.27}
\expandafter\def\csname fm@a8b128@sync\endcsname{1348}
\expandafter\def\csname fm@a8b128@colocate_async\endcsname{1653}
\expandafter\def\csname fm@a8b128@async_2p2\endcsname{1510}
\expandafter\def\csname fm@a8b128@ctrl\endcsname{2409}
\expandafter\def\csname fmx@a8b128@sync\endcsname{1.79}
\expandafter\def\csname fmx@a8b128@colocate_async\endcsname{1.46}
\expandafter\def\csname fmx@a8b128@async_2p2\endcsname{1.59}
\expandafter\def\csname fmb@a8b128\endcsname{1.46}
\expandafter\def\csname fm@a8b256@sync\endcsname{2012}
\expandafter\def\csname fm@a8b256@colocate_async\endcsname{2374}
\expandafter\def\csname fm@a8b256@async_2p2\endcsname{1813}
\expandafter\def\csname fm@a8b256@ctrl\endcsname{3136}
\expandafter\def\csname fmx@a8b256@sync\endcsname{1.56}
\expandafter\def\csname fmx@a8b256@colocate_async\endcsname{1.32}
\expandafter\def\csname fmx@a8b256@async_2p2\endcsname{1.73}
\expandafter\def\csname fmb@a8b256\endcsname{1.32}
\expandafter\def\csname fmdc@a8b256\endcsname{1.20}
\expandafter\def\csname fmds@a8b256\endcsname{1.10}
\expandafter\def\csname fmg@a8b256\endcsname{30}
\expandafter\def\csname fm@h8n64@sync\endcsname{2312}
\expandafter\def\csname fm@h8n64@colocate_async\endcsname{3018}
\expandafter\def\csname fm@h8n64@async_2p2\endcsname{3000}
\expandafter\def\csname fm@h8n64@ctrl\endcsname{4642}
\expandafter\def\csname fmx@h8n64@sync\endcsname{2.01}
\expandafter\def\csname fmx@h8n64@colocate_async\endcsname{1.54}
\expandafter\def\csname fmx@h8n64@async_2p2\endcsname{1.55}
\expandafter\def\csname fmb@h8n64\endcsname{1.54}
\expandafter\def\csname fmdc@h8n64\endcsname{1.28}
\expandafter\def\csname fmds@h8n64\endcsname{1.20}
\expandafter\def\csname fmg@h8n64\endcsname{16}
\expandafter\def\csname fm@h8n128@sync\endcsname{3668}
\expandafter\def\csname fm@h8n128@colocate_async\endcsname{4632}
\expandafter\def\csname fm@h8n128@async_2p2\endcsname{3444}
\expandafter\def\csname fm@h8n128@ctrl\endcsname{6063}
\expandafter\def\csname fmx@h8n128@sync\endcsname{1.65}
\expandafter\def\csname fmx@h8n128@colocate_async\endcsname{1.31}
\expandafter\def\csname fmx@h8n128@async_2p2\endcsname{1.76}
\expandafter\def\csname fmb@h8n128\endcsname{1.31}
\expandafter\def\csname fmdc@h8n128\endcsname{1.16}
\expandafter\def\csname fmds@h8n128\endcsname{1.13}
\expandafter\def\csname fmg@h8n128\endcsname{11}
\expandafter\def\csname fm@h8n256@sync\endcsname{5159}
\expandafter\def\csname fm@h8n256@colocate_async\endcsname{6157}
\expandafter\def\csname fm@h8n256@async_2p2\endcsname{4030}
\expandafter\def\csname fm@h8n256@ctrl\endcsname{7303}
\expandafter\def\csname fmx@h8n256@sync\endcsname{1.42}
\expandafter\def\csname fmx@h8n256@colocate_async\endcsname{1.19}
\expandafter\def\csname fmx@h8n256@async_2p2\endcsname{1.81}
\expandafter\def\csname fmb@h8n256\endcsname{1.19}
\expandafter\def\csname fmdc@h8n256\endcsname{1.10}
\expandafter\def\csname fmds@h8n256\endcsname{1.08}
\expandafter\def\csname fmg@h8n256\endcsname{6}
\expandafter\def\csname fm@a8t64@sync\endcsname{1606}
\expandafter\def\csname fm@a8t64@colocate_async\endcsname{1848}
\expandafter\def\csname fm@a8t64@async_2p2\endcsname{1390}
\expandafter\def\csname fm@a8t64@ctrl\endcsname{2326}
\expandafter\def\csname fmx@a8t64@sync\endcsname{1.45}
\expandafter\def\csname fmx@a8t64@colocate_async\endcsname{1.26}
\expandafter\def\csname fmx@a8t64@async_2p2\endcsname{1.67}
\expandafter\def\csname fmb@a8t64\endcsname{1.26}
\expandafter\def\csname fmdc@a8t64\endcsname{1.23}
\expandafter\def\csname fmds@a8t64\endcsname{1.02}
\expandafter\def\csname fmg@a8t64\endcsname{33}
\expandafter\def\csname fm@a8t128@sync\endcsname{2062}
\expandafter\def\csname fm@a8t128@colocate_async\endcsname{2316}
\expandafter\def\csname fm@a8t128@async_2p2\endcsname{1748}
\expandafter\def\csname fm@a8t128@ctrl\endcsname{2704}
\expandafter\def\csname fmx@a8t128@sync\endcsname{1.31}
\expandafter\def\csname fmx@a8t128@colocate_async\endcsname{1.17}
\expandafter\def\csname fmx@a8t128@async_2p2\endcsname{1.55}
\expandafter\def\csname fmb@a8t128\endcsname{1.17}
\expandafter\def\csname fmdc@a8t128\endcsname{1.15}
\expandafter\def\csname fmds@a8t128\endcsname{1.01}
\expandafter\def\csname fmg@a8t128\endcsname{23}
\expandafter\def\csname fm@h16k64@sync\endcsname{2880}
\expandafter\def\csname fm@h16k64@colocate_async\endcsname{3561}
\expandafter\def\csname fm@h16k64@async_2p2\endcsname{2887}
\expandafter\def\csname fm@h16k64@ctrl\endcsname{4108}
\expandafter\def\csname fmx@h16k64@sync\endcsname{1.43}
\expandafter\def\csname fmx@h16k64@colocate_async\endcsname{1.15}
\expandafter\def\csname fmx@h16k64@async_2p2\endcsname{1.42}
\expandafter\def\csname fmb@h16k64\endcsname{1.15}
\expandafter\def\csname fmdc@h16k64\endcsname{1.12}
\expandafter\def\csname fmds@h16k64\endcsname{1.03}
\expandafter\def\csname fmg@h16k64\endcsname{38}
\expandafter\def\csname fm@h16k128@sync\endcsname{3636}
\expandafter\def\csname fm@h16k128@colocate_async\endcsname{4145}
\expandafter\def\csname fm@h16k128@async_2p2\endcsname{3536}
\expandafter\def\csname fm@h16k128@ctrl\endcsname{4823}
\expandafter\def\csname fmx@h16k128@sync\endcsname{1.33}
\expandafter\def\csname fmx@h16k128@colocate_async\endcsname{1.16}
\expandafter\def\csname fmx@h16k128@async_2p2\endcsname{1.36}
\expandafter\def\csname fmb@h16k128\endcsname{1.16}
\expandafter\def\csname fmdc@h16k128\endcsname{1.14}
\expandafter\def\csname fmds@h16k128\endcsname{1.02}
\expandafter\def\csname fmg@h16k128\endcsname{11}
\expandafter\def\csname fm@h16k256@sync\endcsname{4311}
\expandafter\def\csname fm@h16k256@colocate_async\endcsname{4604}
\expandafter\def\csname fm@h16k256@async_2p2\endcsname{3538}
\expandafter\def\csname fm@h16k256@ctrl\endcsname{5129}
\expandafter\def\csname fmx@h16k256@sync\endcsname{1.19}
\expandafter\def\csname fmx@h16k256@colocate_async\endcsname{1.11}
\expandafter\def\csname fmx@h16k256@async_2p2\endcsname{1.45}
\expandafter\def\csname fmb@h16k256\endcsname{1.11}
\expandafter\def\csname fmdc@h16k256\endcsname{1.10}
\expandafter\def\csname fmds@h16k256\endcsname{1.01}
\expandafter\def\csname fmg@h16k256\endcsname{16}
\expandafter\def\csname fm@rmb64@sync\endcsname{400}
\expandafter\def\csname fm@rmb64@colocate_async\endcsname{422}
\expandafter\def\csname fm@rmb64@async_2p2\endcsname{512}
\expandafter\def\csname fm@rmb64@ctrl\endcsname{1150}
\expandafter\def\csname fmx@rmb64@sync\endcsname{2.87}
\expandafter\def\csname fmx@rmb64@colocate_async\endcsname{2.72}
\expandafter\def\csname fmx@rmb64@async_2p2\endcsname{2.24}
\expandafter\def\csname fmb@rmb64\endcsname{2.24}
\expandafter\def\csname fmdc@rmb64\endcsname{1.99}
\expandafter\def\csname fmds@rmb64\endcsname{1.37}
\expandafter\def\csname fmg@rmb64\endcsname{3}
\expandafter\def\csname fm@rmb128@sync\endcsname{664}
\expandafter\def\csname fm@rmb128@colocate_async\endcsname{782}
\expandafter\def\csname fm@rmb128@async_2p2\endcsname{953}
\expandafter\def\csname fm@rmb128@ctrl\endcsname{1634}
\expandafter\def\csname fmx@rmb128@sync\endcsname{2.46}
\expandafter\def\csname fmx@rmb128@colocate_async\endcsname{2.09}
\expandafter\def\csname fmx@rmb128@async_2p2\endcsname{1.71}
\expandafter\def\csname fmb@rmb128\endcsname{1.71}
\expandafter\def\csname fmdc@rmb128\endcsname{1.56}
\expandafter\def\csname fmds@rmb128\endcsname{1.34}
\expandafter\def\csname fmg@rmb128\endcsname{0}
\expandafter\def\csname fm@rmb256@sync\endcsname{1260}
\expandafter\def\csname fm@rmb256@colocate_async\endcsname{1300}
\expandafter\def\csname fm@rmb256@async_2p2\endcsname{1026}
\expandafter\def\csname fm@rmb256@ctrl\endcsname{2732}
\expandafter\def\csname fmx@rmb256@sync\endcsname{2.17}
\expandafter\def\csname fmx@rmb256@colocate_async\endcsname{2.10}
\expandafter\def\csname fmx@rmb256@async_2p2\endcsname{2.66}
\expandafter\def\csname fmb@rmb256\endcsname{2.10}
\expandafter\def\csname fmdc@rmb256\endcsname{1.60}
\expandafter\def\csname fmds@rmb256\endcsname{1.32}
\expandafter\def\csname fmg@rmb256\endcsname{0}
\expandafter\def\csname fm@amt64@sync\endcsname{1475}
\expandafter\def\csname fm@amt64@colocate_async\endcsname{1934}
\expandafter\def\csname fm@amt64@async_2p2\endcsname{1548}
\expandafter\def\csname fm@amt64@ctrl\endcsname{2510}
\expandafter\def\csname fmx@amt64@sync\endcsname{1.70}
\expandafter\def\csname fmx@amt64@colocate_async\endcsname{1.30}
\expandafter\def\csname fmx@amt64@async_2p2\endcsname{1.62}
\expandafter\def\csname fmb@amt64\endcsname{1.30}
\expandafter\def\csname fmdc@amt64\endcsname{1.20}
\expandafter\def\csname fmds@amt64\endcsname{1.08}
\expandafter\def\csname fmg@amt64\endcsname{44}
\expandafter\def\csname fm@amt128@sync\endcsname{2114}
\expandafter\def\csname fm@amt128@colocate_async\endcsname{2542}
\expandafter\def\csname fm@amt128@async_2p2\endcsname{1985}
\expandafter\def\csname fm@amt128@ctrl\endcsname{3448}
\expandafter\def\csname fmx@amt128@sync\endcsname{1.63}
\expandafter\def\csname fmx@amt128@colocate_async\endcsname{1.36}
\expandafter\def\csname fmx@amt128@async_2p2\endcsname{1.74}
\expandafter\def\csname fmb@amt128\endcsname{1.36}
\expandafter\def\csname fmdc@amt128\endcsname{1.29}
\expandafter\def\csname fmds@amt128\endcsname{1.05}
\expandafter\def\csname fmg@amt128\endcsname{24}
\expandafter\def\csname fm@amt256@sync\endcsname{2802}
\expandafter\def\csname fm@amt256@colocate_async\endcsname{2962}
\expandafter\def\csname fm@amt256@async_2p2\endcsname{2150}
\expandafter\def\csname fm@amt256@ctrl\endcsname{4553}
\expandafter\def\csname fmx@amt256@sync\endcsname{1.63}
\expandafter\def\csname fmx@amt256@colocate_async\endcsname{1.54}
\expandafter\def\csname fmx@amt256@async_2p2\endcsname{2.12}
\expandafter\def\csname fmb@amt256\endcsname{1.54}
\expandafter\def\csname fmdc@amt256\endcsname{1.50}
\expandafter\def\csname fmds@amt256\endcsname{1.03}
\expandafter\def\csname fmg@amt256\endcsname{4}
\expandafter\def\csname fm@hmb64@sync\endcsname{1576}
\expandafter\def\csname fm@hmb64@colocate_async\endcsname{2797}
\expandafter\def\csname fm@hmb64@async_2p2\endcsname{2661}
\expandafter\def\csname fm@hmb64@ctrl\endcsname{3140}
\expandafter\def\csname fmx@hmb64@sync\endcsname{1.99}
\expandafter\def\csname fmx@hmb64@colocate_async\endcsname{1.12}
\expandafter\def\csname fmx@hmb64@async_2p2\endcsname{1.18}
\expandafter\def\csname fmb@hmb64\endcsname{1.12}
\expandafter\def\csname fmdc@hmb64\endcsname{0.99}
\expandafter\def\csname fmds@hmb64\endcsname{1.13}
\expandafter\def\csname fmg@hmb64\endcsname{40}
\expandafter\def\csname fm@hmb128@sync\endcsname{3091}
\expandafter\def\csname fm@hmb128@colocate_async\endcsname{4054}
\expandafter\def\csname fm@hmb128@async_2p2\endcsname{3533}
\expandafter\def\csname fm@hmb128@ctrl\endcsname{4855}
\expandafter\def\csname fmx@hmb128@sync\endcsname{1.57}
\expandafter\def\csname fmx@hmb128@colocate_async\endcsname{1.20}
\expandafter\def\csname fmx@hmb128@async_2p2\endcsname{1.37}
\expandafter\def\csname fmb@hmb128\endcsname{1.20}
\expandafter\def\csname fmdc@hmb128\endcsname{1.11}
\expandafter\def\csname fmds@hmb128\endcsname{1.08}
\expandafter\def\csname fmg@hmb128\endcsname{31}
\expandafter\def\csname fm@hmb256@sync\endcsname{4692}
\expandafter\def\csname fm@hmb256@colocate_async\endcsname{5414}
\expandafter\def\csname fm@hmb256@async_2p2\endcsname{4213}
\expandafter\def\csname fm@hmb256@ctrl\endcsname{6505}
\expandafter\def\csname fmx@hmb256@sync\endcsname{1.39}
\expandafter\def\csname fmx@hmb256@colocate_async\endcsname{1.20}
\expandafter\def\csname fmx@hmb256@async_2p2\endcsname{1.54}
\expandafter\def\csname fmb@hmb256\endcsname{1.20}
\expandafter\def\csname fmdc@hmb256\endcsname{1.14}
\expandafter\def\csname fmds@hmb256\endcsname{1.05}
\expandafter\def\csname fmg@hmb256\endcsname{17}
\expandafter\def\csname fm@a8t256@sync\endcsname{2349}
\expandafter\def\csname fm@a8t256@colocate_async\endcsname{2467}
\expandafter\def\csname fm@a8t256@async_2p2\endcsname{1514}
\expandafter\def\csname fm@a8t256@ctrl\endcsname{3018}
\expandafter\def\csname fmx@a8t256@sync\endcsname{1.28}
\expandafter\def\csname fmx@a8t256@colocate_async\endcsname{1.22}
\expandafter\def\csname fmx@a8t256@async_2p2\endcsname{1.99}
\expandafter\def\csname fmb@a8t256\endcsname{1.22}
\expandafter\def\csname fmdc@a8t256\endcsname{1.21}
\expandafter\def\csname fmds@a8t256\endcsname{1.01}
\expandafter\def\csname fmg@a8t256\endcsname{25}
\expandafter\def\csname fmg@a8b64\endcsname{62}
\expandafter\def\csname fmg@a8b128\endcsname{24}
\makeatother
\newcommand{\HeadBestLo}{1.11}
\newcommand{\HeadBestHi}{2.24}
\newcommand{\HeadColocLo}{1.11}
\newcommand{\HeadColocHi}{2.72}
\newcommand{\HeadDisaggLo}{1.18}
\newcommand{\HeadDisaggHi}{2.66}
\newcommand{\HeadSyncLo}{1.19}
\newcommand{\HeadSyncHi}{2.87}
\newcommand{\HeadRows}{24}
\newcommand{\HeadBaseLo}{1.27}
\newcommand{\HeadBaseHi}{2.24}
\newcommand{\HeadThinkLo}{1.11}
\newcommand{\HeadThinkHi}{1.54}
\newcommand{\HeadSwitchBaseLo}{1.07}
\newcommand{\HeadSwitchBaseHi}{1.37}
\newcommand{\HeadSwitchThinkLo}{1.01}
\newcommand{\HeadSwitchThinkHi}{1.13}
\newcommand{\IntroRCtrlTok}{2076}
\newcommand{\IntroRColocTok}{1457}
\newcommand{\IntroRDisaggTok}{1247}
\newcommand{\IntroRSyncTok}{1199}
\newcommand{\IntroRColocRatio}{1.42}
\newcommand{\IntroRDisaggRatio}{1.67}
\newcommand{\IntroRSyncRatio}{1.73}
\newcommand{\IntroRSyncGenPct}{56}
\newcommand{\IntroRSyncLearnerPct}{39}
\newcommand{\IntroRSyncSwitchPct}{5}
\newcommand{\IntroRSyncLearnerS}{66}
\newcommand{\IntroRDisaggLearnerS}{147}
\newcommand{\BgRSyncGenS}{96}
\newcommand{\BgRSyncSwitchS}{8.9}
\newcommand{\BgRColocGenS}{62}
\newcommand{\BgRColocLearnerS}{70}

